Word-level confidence estimation for RNN transducers

Confidence estimate is an often requested feature in applications such as medical transcription where errors can impact patient care and the confidence estimate could be used to alert medical professionals to verify potential errors in recognition. In this paper, we present a lightweight neural confidence model tailored for Automatic Speech Recognition (ASR) system with Recurrent Neural Network Transducers (RNN-T). Compared to other existing approaches, our model utilizes: (a) the time information associated with recognized words, which reduces the computational complexity, and (b) a simple and elegant trick for mapping between sub-word and word sequences. The mapping addresses the non-unique tokenization and token deletion problems while amplifying differences between confusable words. Through extensive empirical evaluations on two different long-form test sets, we demonstrate that the model achieves a performance of 0.4 Normalized Cross Entropy (NCE) and 0.05 Expected Calibration Error (ECE). It is robust across different ASR configurations, including target types (graphemes vs. morphemes), traffic conditions (streaming vs. non-streaming), and encoder types. We further discuss the importance of evaluation metrics to reflect practical applications and highlight the need for further work in improving Area Under the Curve (AUC) for Negative Precision Rate (NPV) and True Negative Rate (TNR).

==> outline.tex <==
\begin{itemize}
\item \textbf{MOTIVATION}: Confidence score at both utterance level and word level is useful for many speech applications. However we can't directly use the posteriors from the neural ASR models since they are spiky and over confident. 
\item Analyze some potential reasons why RNN-T model has a skewed posterior.
\begin{enumerate}
    \item Maybe because of the LM inside of a RNN-T. 
    \item Besides, the CE objective could always be minimized even it has predicted the right class. 
\end{enumerate}

\item \textbf{BACKGROUND AND TASK DEFINITION}: Although there have been some work recently on neural confidence for E2E ASR model, there's still no neural confidence for a RNN-T ASR directly. Therefore we show a neural confidence model for RNN-T.
\begin{enumerate}
    \item Existing calibration work:
    \begin{enumerate}
    \item Temperature scaling
    \item Pairwise mapping
    \item regularization
    \item deep ensemble
    \item MC dropout
    \end{enumerate}
    \item David and Qiujia's papers are focusing on utterance level confidence score.
    \item Besides, their works mostly focus on short utterance.
    \item We report confidence score for all punctuations and speaker labels.
    \item Additional, their models are more designed for LAS, while ours are for RNN-T.
    \begin{enumerate}
    \item RNN-T has additional emit time field which we can make use of.
    \item We can't directly use joint layer output.
\end{enumerate}
\end{enumerate}
\item \textbf{MODEL ARCHITECTURE}: We show Model architectures. For example, we hard-attend to acoustic frame using the emit time (this is not given in LAS model). We use a sliding window around the emit time to select acoustic model output. Different loss types. 

Input features: LM emb, emit time, AM output.
why we didn't use joint layer output?

\item Data augmentations since ASR models are typically very strong. 
\begin{enumerate}
    \item WER being low means harder to train confidence model.
    \item Up-sample wrong ASR prediction.  
    \item N-best hypothesis
    \item Cutout.
    \item Stabilize the model by data augumentation. Very useful.
\end{enumerate}

\item Evaluation metrics for confidence model. 
\begin{enumerate}
\item NCE
\item ECE
\item AUC - Downstream applications want to detect as many wrong words as possible but not to sacrifice sensitivity. We show that although NCE/ECE/AUC under ROC and PRC are all very good, we may not easily find the operating point on the NPV TNR curve. The current best AUC is only 0.6 for dictation case. 
\item KL divergence, Thresholded accuracy, Precision, Recall, and F-score
\end{enumerate}

\item Use a small trick to avoid token deletion problem. Align at word but predict at token.


\item \textbf{DATASET}:
\begin{itemize}
\item Librispeech (public dataset so that we can compare to published works.
\item Medical dictations.
\item Medical conversations.
\end{itemize}

\item \textbf{EXPERIMENTS}:

\begin{itemize}
\item Model backbone. transformer less overfits than LSTM even given the same model size. Dense is absolutely bad. Need to learn contextual dependency. 
\item Loss (focal, xent, crf)
\item How to pick up frame, attention. 
\begin{enumerate}
    \item Didn't see attention works well.
    \item The best case is to feed accurate emit time for each token to the confidence model.
    \item Another extreme case is to use attention to select AM output without using emit time at all. 
    \item The large the window size is, the worse performance is.
\end{enumerate}
\item Fuzzy alignment used for mitigate the sensitivity to emit time. No influence on model performance. 
\end{itemize}

\item Observed issues
\begin{itemize}
\item model being very sensitive to emit time. Does it overfit on emit?
\item word deletion issue. Span prediction model. 
\end{itemize}

\end{itemize}


\textbf{MISC}:
We can't make a conclusion that morpheme model is better than grapheme model / Uni is better than bi / LSTM based is better than transformer based.



\textbf{Missing Experiments}:
\begin{itemize}

\item Replace the CRF with RNN.
\item Use forward and backward for output dependency.
\item Have a RNN-T on top of transformer to replace CRF.
\item Maybe useful for decay the alpha and gamma.
\item CTC model to demonstrate LM in RNN-T being an issue. 
\item Mimic deep ensemble. Train N different confidence models with different model architectures.

\end{itemize}
